Tensor Network Space-Time Spectral Collocation Method for Time Dependent Convection-Diffusion-Reaction Equations

Emerging tensor network techniques for solutions of Partial Differential Equations (PDEs), known for their ability to break the curse of dimensionality, deliver new mathematical methods for ultrafast numerical solutions of high-dimensional problems. Here, we introduce a Tensor Train (TT) Chebyshev spectral collocation method, in both space and time, for solution of the time dependent convection-diffusion-reaction (CDR) equation with inhomogeneous boundary conditions, in Cartesian geometry. Previous methods for numerical solution of time dependent PDEs often use finite difference for time, and a spectral scheme for the spatial dimensions, which leads to slow linear convergence. Spectral collocation space-time methods show exponential convergence, however, for realistic problems they need to solve large four-dimensional systems. We overcome this difficulty by using a TT approach as its complexity only grows linearly with the number of dimensions. We show that our TT space-time Chebyshev spectral collocation method converges exponentially, when the solution of the CDR is smooth, and demonstrate that it leads to very high compression of linear operators from terabytes to kilobytes in TT-format, and tens of thousands times speedup when compared to full grid space-time spectral method. These advantages allow us to obtain the solutions at much higher resolutions.

==> ex_shared.tex <==
% Hey Emacs, this is -*-latex-*-

% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
\input{ttdefs_SIAM.tex}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{TN Space-Time Spectral Method Convection-Diffusion-Reaction
  Equations}{ D. Adak, D.P. Truong, G. Manzini, K.\O. Rasmussen,
  B. S. Alexandrov}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Tensor Network Space-Time Spectral Collocation Method for
  Time-Dependent Convection-Diffusion-Reaction Equations
\thanks{Submitted to the editors DATE.\funding{This work was funded by
    the LDRD-DR Program of the Los Alamos National Laboratory}}}
  
% Authors: full names plus addresses.
\author{
  Dibyendu Adak\thanks{Theoretical Division, Los Alamos National Laboratory, Los
    Alamos, NM 87545, USA}\and
  Duc P. Truong\footnotemark[2]\and
  Gianmarco Manzini\footnotemark[2]\and
  Kim \O. Rasmussen\footnotemark[2]\and
  Boian S. Alexandrov\footnotemark[2]
}

%%   \thanks{Theoretical Division, Los Alamos National Laboratory,
%%     Los Alamos, NM 87545, USA}
%%     Los Alamos National Laboratory
%%     (\email{dadak@lanl.gov}, \url{http://www.imag.com/\string~ddoe/}).}
%% \and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
%%   (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
%% \and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> sec1_intro.tex <==
\section{Introduction}
\label{sec1:introduction}

Solving realistic problems in physics, chemistry, and engineering
often require numerical solutions of high-dimensional partial
differential equations (PDEs).
%%
PDE discretization leads to an exponential increase of the number of
grid points with the dimension of the problem, often making numerical
solution infeasible.
%%
This \emph{curse of dimensionality}~\cite{bellman1966dynamic} poses a
fundamental challenge to multidimensional numerical computation, which
even exascale high-performance computing cannot overcome.
%%
Recently, \emph{tensor networks} (\TNs{})~\cite{bachmayr2016tensor}
have emerged as a promising approach to mitigate or remove the curse
of dimensionality.
%%
\TNs{} partition high-dimensional data into smaller, manageable blocks of
data by approximating high-dimensional arrays with networks of
low-dimensional tensors.
%%0
Tensor factorization formats like Canonical Polyadic Decomposition,
Hierarchical Tucker decomposition~\cite{kolda2009tensor}, and Tensor
Train~\cite{oseledets2011tensor} can be viewed as tensor networks.
%%
Originally developed in theoretical physics, now \TNs{} show promise
for accurate and efficient numerical solutions of high-dimensional
PDEs.
%%
\TNs{} provide a strategy, that we will call \emph{tensorization}, for
efficiently representing the two main components of numerical
algorithms for high-dimensional PDEs: grid functions capturing
function values at grid nodes, and discrete operators approximating
differential operators.
%%
Specific examples solved recently using \TNs{} include the Poisson
\cite{kazeev2012low}, Schr{\"o}dinger \cite{gelss2022solving},
Poisson-Boltzmann \cite{benner2021regularization}, Smoluchowski
\cite{matveev2016tensor, manzini2021nonnegative}, Maxwell
\cite{manzini2023tensor}, Vlasov-Poisson/Maxwell
\cite{ye2022quantum,ye2023quantized,kormann2015semi}, neutron
transport equations \cite{truong2023tensor}, etc.

In this work, we consider the \emph{time-dependent,
convection-diffusion-reaction (CDR) equation}.
%%
This model equation holds vital significance across numerous physical
and engineering systems by governing the coupled transport and
transformation of scalars via diffusion, advection, and reactive
processes \cite{bejan2013convection,chandrasekhar1943stochastic}.
%%
The CDR equation enables quantitative descriptions of heat transfer,
mass transfer, fluid dynamics, and chemical interactions in complex
settings from microscale processing to atmospheric modeling.
%%
Numerical methods for the multidimensional CDR equation also
constitute a major research area given the equation’s utility spanning
such a vast range of transport phenomena critical to climate modeling,
energy systems, biomedical systems, materials synthesis, and related
domains central to technology
innovation~\cite{stocker2011introduction,bird1960we,doi1988theory}.

Solving realistic time-dependent, three-dimensional (3D) CDR equations
poses substantial computational demands.
%%
Classical methods like finite differences and finite volumes rely on
discrete approximation of differential operators on a grid and they
require very fine grids if accurate solutions are needed
\cite{evans2012numerical}.
%%
Discretizing the CDR equation on a 3D spatial grid and applying
different temporal schemes leads to very large-scale linear systems
requiring iterative solvers and parallel computing, which for four
(one temporal and three spatial) dimensions problems are often
infeasible.
%%
That is why, \emph{spectral collocation methods} can be considered and
proven to be more efficient.

A spectral collocation method approximates the CDR solution using
high-order polynomial interpolants (e.g., Legendre, Chebyshev, etc.)
through collocation points.
%%
The spatial interpolation error decreases exponentially with the
polynomial degree if the solution to be numerically approximated is
sufficiently regular in space, thus providing the \emph{exponential
convergence}.
%%
However, the standard approach for time-dependent PDEs couples
spectral discretization of spatial derivatives with low-order finite
difference temporal derivatives and the temporal error dominates the
accurate spectral spatial resolution.
%%
Ideally, the accuracy of the time integration should match that of the
spatial spectral approximation.
%%
Recent methods address this time-stepping limitation in various ways
to better leverage the precision of spectral representations by
including space-time spectral collocation methods.
%%
The introduced space-time spectral collocation methods have
demonstrated exponential convergence in both the spatial and temporal
dimensions when applied to solutions of the heat equation that are
sufficiently smooth.
%%
This points to the possibility of realizing numerical solutions that
fully leverage the precision of spectral representations in space and
time simultaneously.
%%
However, for realistic CDR problems demanding high accuracy, the
space-time formulation requires solving prohibitively large systems
arising from the four-dimensional discretization.
%%
Thus, the curse of dimensionality poses a significant challenge for
space-time spectral methods for CDR equations, with computational
complexity growing exponentially with problem size.

Here, we introduce a new \TTf{} spectral collocation space-time
(\TTf{}-\SCST{}) method that restricts complexity growth from
exponential to linear in the number of dimensions.
%%
We demonstrate that \TTf{}-SCST for CDR equations maintains spectral
accuracy, while enabling tens of thousands times acceleration and
terabyte-to-kilobyte memory compression compared to conventional
space-time spectral discretizations.
%%
Manufactured solutions verify that the exponential convergence is
preserved.
%%
The \TTf{} factorization hence makes viable extremely precise space-time
simulations of CDR physics with inhomogeneous boundary conditions,
that would otherwise be intractable with standard
techniques.
%%
Although, for simplicity, our results are demonstrated only on
four-dimensional CDRs, they are also valid for higher-dimensional
cases.
%%
The introduced \TTf{}-SCST, therefore, paves the way for efficient
numerical modeling of large high-dimensional systems with spectral
precision.

The outline of the paper is as follows.
%%
In Section~\ref{sec:spacetimeapproach}, we review some basic concepts
for space-time collocation methods, introduce the discretization and
its matrix formulation that leads to a linear system.
%%
In Section~\ref{sec:Tensor-Networks}, we review the tensor notations
and definitions of the \TTf{}-formart, and the \TTf{}-matrix format for linear
operators.
%%
In Section~\ref{tensorization}, we present our \TTf{} design of the
numerical solution of the CDR equation and introduce our algorithms in
tensor train format.
%%
In Section~\ref{results}, we present our numerical results and assess
the performance of our method.
%%
In Section~\ref{conclusions}, we offer our final remarks and discusses
possible future work.
%%
For completeness, part of the details of the CDR tensorization
approach are in a final appendix.












